Decentralized Gradient-Free Methods for Stochastic Non-Smooth Non-Convex Optimization

We consider decentralized gradient-free optimization of minimizing Lipschitz continuous functions that satisfy neither smoothness nor convexity assumption. We propose two novel gradient-free algorithms, the Decentralized Gradient-Free Method (DGFM) and its variant, the Decentralized Gradient-Free Method$^+$ (DGFM$^{+}$). Based on the techniques of randomized smoothing and gradient tracking, DGFM requires the computation of the zeroth-order oracle of a single sample in each iteration, making it less demanding in terms of computational resources for individual computing nodes. Theoretically, DGFM achieves a complexity of $\mathcal O(d^{3/2}\delta^{-1}\varepsilon ^{-4})$ for obtaining an $(\delta,\varepsilon)$-Goldstein stationary point. DGFM$^{+}$, an advanced version of DGFM, incorporates variance reduction to further improve the convergence behavior. It samples a mini-batch at each iteration and periodically draws a larger batch of data, which improves the complexity to $\mathcal O(d^{3/2}\delta^{-1} \varepsilon^{-3})$. Moreover, experimental results underscore the empirical advantages of our proposed algorithms when applied to real-world datasets.

==> abstract.tex <==
We consider decentralized gradient-free optimization of a general class of Lipschitz continuous functions that satisfy neither smoothness nor convexity assumption. We propose two novel gradient-free algorithms, the Decentralized Gradient-Free Method (DGFM) and its variant, the Decentralized Gradient-Free Method$^+$ (DGFM$^{+}$).
Based on the techniques of randomized smoothing and gradient tracking, DGFM requires the computation of the zeroth-order oracle of a single sample in each iteration, making it less demanding in terms of computational resources for individual computing nodes. Theoretically, DGFM achieves a complexity of $O(\delta^{-1}\varepsilon^{-4})$ for obtaining the $(\delta,\varepsilon)$-Goldstein stationary condition. 
DGFM$^{+}$, an advanced version of DGFM,  incorporates variance reduction to further improve the convergence performance. It samples a mini-batch at each iteration and periodically draws a larger batch of data, which improves the complexity to $O(\delta^{-1}\varepsilon^{-3})$, aligning with the state-of-the-art result for zeroth-order non-smooth non-convex optimization in the centralized setting. Moreover, experimental results underscore the empirical advantages of our proposed algorithms when applied to real-world datasets.

==> numerical.tex <==




% % Table generated by Excel2LaTeX from sheet 'summary'
% \begin{table}[htbp]
%   \centering
%   \caption{Descriptions of datasets used in our experiment}
%     \begin{tabular}{crr|crr}
%     \toprule
%     Dataset & \multicolumn{1}{c}{n} & \multicolumn{1}{c|}{d} & Dataset & \multicolumn{1}{c}{n } & \multicolumn{1}{c}{d} \\
%     \midrule
%     a9a   & 32561 & 123   & w8a   & 49749 & 300 \\
%     HIGGS & 1.1E+07 & 28    & covtype & 581012 & 54 \\
%     rcv   & 20242 & 47236 & SUSY  & 5.0E+06 & 18 \\
%     ijcnn1 & 49990 & 22    & skin\_nonskin & 245,057 & 3 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%




% \begin{table*}[htp]
%   \centering
%   \caption{Descriptions of datasets used in our experiment}
%   \vspace{-1.0em}
%     \begin{tabular}{crrrrrrrrr}
%     \toprule
%     Dataset & a9a   & HIGGS & rcv & ijcnn1 & w8a   & covtype  &   SUSY  & skin\_nonskin  \\
%     \midrule
%     $n$     & 32,561 & 11,000,000 & 20,242 & 49,990 & 49,749 & 581,012  &   5,000,000 & 245,057  \\
%     $d$     & 123  & 28  & 47,236 & 22  & 300   & 54          & 18    & 3     \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:dataset_descript}%
% \end{table*}%
\section{Numerical Study}
In this section, we show the empirical performance of  {\dgfmlin} and 
{\dgfm}  via some numerical experiments.

\subsection{Nonconvex SVM with Capped-$\ell_1$ Penalty}
\textbf{Data: }We evaluate our proposed algorithms using several standard datasets in LIBSVM~\cite{chang2011libsvm}, which are described in Table~\ref{tab:dataset_descript}. The feature vectors of all datasets are normalized before optimization.
% Table generated by Excel2LaTeX from sheet 'summary'
\vspace{-0.5em}
\begin{table}[htbp]
  \centering
  \fontsize{9}{11}\selectfont
    \setlength{\tabcolsep}{0.8mm}
    \begin{tabular}{crr|crr}
    \toprule
    Dataset & \multicolumn{1}{c}{$n$}     & \multicolumn{1}{c|}{$d$}     & Dataset & \multicolumn{1}{c}{$n$}     & \multicolumn{1}{c}{$d$} \\
    \midrule
    a9a   & 32,561 & 123   & w8a   & 49,749 & 300 \\
    HIGGS & 11,000,000 & 28    & covtype & 581,012 & 54 \\
    rcv   & 20,242 & 47,236 & SUSY  & 5,000,000 & 18 \\
    ijcnn1 & 49,990 & 22    & skin\_nonskin & 245,057 & 3 \\
    \bottomrule
    \end{tabular}%
    \vspace{-0.5em}
  \caption{\label{tab:dataset_descript}Descriptions of datasets used in our experiments}
  \vspace{-0.5em}
\end{table}%

\noindent\textbf{Model: }We consider the nonconvex penalized SVM with capped-$\ell_1$ regularizer~\cite{zhang2010analysis}. The model aims at training a binary classifier $x\in \mbb R^d$ on the training data $\{a_i,b_i\}_{i=1}^n$, where $a_i\in \mbb R^d$ and $b_i\in \{1,-1\}$ are the feature of the $i-$th sample and its label, respectively. For {\dgfm} and {\dgfmlin}, the objective function can be written as
\vspace{-0.5em}
\begin{equation}
    \begin{aligned}
        \min_{x\in \mbb R^d} f(x)&=\tfrac{1}{m}\tsum_{i=1}^m f^{i}(x),
    \end{aligned}
\end{equation}
where $f^{i}(x)=\tfrac{1}{n_i}\tsum_{j=1}^{n_i} \ell(b_i^j (a_i^j)^{\top}x)+r(x)$, $\ell(x)=\max\{1-x,0 \allowbreak \}\allowbreak,r(x)\allowbreak=\lambda \allowbreak \tsum_{j=1}^d \allowbreak \min \allowbreak \{\abs{x_j}\allowbreak,\alpha\}$, $n=\tsum_{i=1}^{m}n_i$ and $\lambda,\alpha>0$. Similar to~\cite{chen2023faster}, we take $\lambda = 10^{-5}/n$ and $\alpha=2$.

\noindent\textbf{Network topology:} We consider a simple ring-based topology of the communication network. We set the number of worker nodes to $m=20$. The setting can be found in~\cite{xian2021faster}.
% \begin{equation}
% A(k)\equiv A=\left[\begin{array}{ccccc}
% \tfrac{1}{3} & \tfrac{1}{3} &  &  & \tfrac{1}{3}\\
% \tfrac{1}{3} & \tfrac{1}{3} & \tfrac{1}{3}\\
%  & \tfrac{1}{3} & \tfrac{1}{3} & \ddots\\
%  &  & \ddots & \ddots & \tfrac{1}{3}\\
% \tfrac{1}{3} &  &  & \tfrac{1}{3} & \tfrac{1}{3}
% \end{array}\right]\label{eq:mixing_matrix}
% \end{equation}


\noindent\textbf{Performance measures:} We measure the performance of the decentralized algorithms by the decrease of the global cost function value $f(\bar{x})$, to which we refer as loss versus zeroth-order gradient calls.


\noindent\textbf{Comparison:} We compare the proposed {\dgfmlin} and {\dgfm} with GFM~\cite{lin2022gradient} and GFM$^{+}$~\cite{chen2023faster}. Throughout all the experiments, we set $\delta = 0.001$ and tune the stepsize $\eta$ from $\{0.0005, 0.001, 0.005, 0.01\}$ for all four algorithms and $b^{\prime}$ from $\{10,100,500\}$, $T$ from $\{10,50,100\}$ for {\dgfm} and GFM$^{+}$, $\mcal{T}$ from $\{1,5,10\}$ for {\dgfm}, $m=20$ for two decentralized algorithms.  We run all the algorithms with the same number of calls to the zeroth-order oracles. We plot the average of five runs in Figure~\ref{fig:res}.
% We executed each of the four algorithms once, using five different random seeds for each dataset, and presented the results in Figure~\ref{fig:res}. 


% In most experiments, it can be observed that our decentralized algorithms have significant advantages compared to the corresponding serial algorithms. Both \dgfmlin{} and \dgfm{} exhibit a faster rate of convergence and demonstrates strong stability (much smoother converging curves). This result further confirms our theoretical analysis of \dgfmlin{} and \dgfm{}.  Moreover, in testcases with  a larger sample size (SUSY, HIGGS), {\dgfm} often demonstrates significantly faster convergence than \dgfmlin{}. This result further confirms the theoretical advantage of the variance reduction technique and our convergence rate results. 
In most of the experiments we conducted, our decentralized algorithms significantly outperform their serial counterparts. While DGFM sometimes exhibits slow convergence due to high consensus error, {\dgfm} consistently demonstrates more robust performance and often achieves the best results. In larger sample size test cases (SUSY, HIGGS), {\dgfm} often demonstrates notably faster convergence than \dgfmlin{}.  These outcomes further corroborate our theoretical analysis of \dgfmlin{} and \dgfm{}.
Additionally, we note that both {\dgfm} and GFM$^{+}$ have exhibited significantly stable performance, as seen in their smoother convergence curves, while DGFM and GFM show more fluctuation. This observation aligns with the theoretical advantage offered by the variance reduction technique.
\begin{figure*}[ht]
\begin{centering}
\begin{minipage}[t]{0.45\columnwidth}%
\includegraphics[width=4.5cm]{fig/a9a.pdf}%
\end{minipage}\hfill
\begin{minipage}[t]{0.45\columnwidth}%
\includegraphics[width=4.5cm]{fig/HIGGS.pdf}%
\end{minipage}\hfill
\begin{minipage}[t]{0.45\columnwidth}%
\includegraphics[width=4.5cm]{fig/rcv.pdf}%
\end{minipage}\hfill
\begin{minipage}[t]{0.45\columnwidth}%
\includegraphics[width=4.5cm]{fig/ijcnn.pdf}%  
\end{minipage}\hfill

\begin{minipage}[t]{0.45\columnwidth}%
\includegraphics[width=4.5cm]{fig/w8a.pdf}% 
\end{minipage}\hfill
\begin{minipage}[t]{0.45\columnwidth}%
\includegraphics[width=4.5cm]{fig/covtype.pdf}%    
\end{minipage}\hfill
\begin{minipage}[t]{0.45\columnwidth}%
\includegraphics[width=4.5cm]{fig/SUSY.pdf}%
\end{minipage}\hfill
\begin{minipage}[t]{0.45\columnwidth}%
\includegraphics[width=4.5cm]{fig/skin_nonskin.pdf}%    
\end{minipage}\hfill
\\
\vspace{-0.8em}
\begin{center}
    \begin{minipage}[t]{1\columnwidth}%
    \includegraphics[width=10cm]{fig/legend.pdf}
\end{minipage}
\end{center}
\end{centering}
\vspace{-1.2em}
\caption{\label{fig:res}Comparison of convergence performance. $y$-axis: objective function value; $x$-axis:  number of calls to the zeroth-order oracle.}
\end{figure*}







\begin{figure*}[ht]
\begin{centering}
\begin{minipage}[t]{0.4\columnwidth}%
\includegraphics[width=4.5cm]{fig/fashion_train.pdf}%
\end{minipage}\hfill
\begin{minipage}[t]{0.4\columnwidth}%
\includegraphics[width=4.5cm]{fig/fashion_test.pdf}%
\end{minipage}\hfill
\begin{minipage}[t]{0.4\columnwidth}%
\includegraphics[width=4.5cm]{fig/mnist_train.pdf}%
\end{minipage}\hfill
\begin{minipage}[t]{0.4\columnwidth}%
\includegraphics[width=4.5cm]{fig/mnist_test.pdf}%  
\end{minipage}\hfill
% \begin{center}
%     \begin{minipage}[t]{1\columnwidth}%
%     \includegraphics[width=10cm]{fig/legend.pdf}
% \end{minipage}
% \end{center}
\end{centering}
\vspace{-1.2em}
\caption{\label{fig:res_attack}Comparison of attack performance. $y$-axis: accuracy after attacking; $x$-axis:  number of calls to the zeroth-order oracle.}
\end{figure*}


\subsection{Universal Attack}
We consider the black-box adversarial attack on image classification with LeNet~\cite{lecun1998gradient}. Our objective is to discover a universal adversarial perturbation~\cite{moosavi2017universal}. When applied to the original image, this perturbation induces misclassification in machine learning models while remaining inconspicuous to human observers. Network topology and Performance measures are the same as in the previous experiment. However, we set $m=8$ for two decentralized algorithms here.
\vspace{-0.5em}
\begin{table}[htbp]
  \centering
  \setlength{\tabcolsep}{0.8mm}
    \begin{tabular}{crrrr}
    \toprule
    \multirow{2}[4]{*}{Dataset} & \multicolumn{2}{c}{Fashion-MNIST} & \multicolumn{2}{c}{MNIST} \\
\cmidrule{2-5}          & \multicolumn{1}{c}{Training} & \multicolumn{1}{c}{Test}  & \multicolumn{1}{c}{Training} & \multicolumn{1}{c}{Test} \\
    \midrule
    DGFM  & \textbf{65.66}(\textbf{0.88}) & \textbf{65.22}(1.07) & 71.92(1.56) & 73.18(1.21) \\
    DGFM$^+$ & 66.46(1.80) & 66.14(2.03) & \textbf{70.62}(2.47) & \textbf{71.42}(2.50) \\
    GFM   & 66.86(0.90) & 66.64(\textbf{1.02}) & 73.20(\textbf{0.41}) & 73.66(\textbf{0.55}) \\
    GFM$^{+}$ & 69.92(2.67) & 69.62(2.63) & 76.64(3.29) & 77.52(3.29) \\
    \bottomrule
    \end{tabular}%
    \vspace{-0.5em}
  \caption{\label{tab:accuracy_attack}Attacking result (Accuracy/std\%)}
  \vspace{-0.5em}
\end{table}%

\noindent\textbf{Data: }We evaluate our proposed algorithms using two standard datasets, {\mnist} and {\fashion}.

\noindent\textbf{Model: }The problem can be formulated as the following nonsmooth nonconvex problem:
\vspace{-0.5em}
\begin{equation}
    \text{min}_{\norm{\zeta}_{\infty}\leq \kappa} \tfrac{1}{m}\tsum_{i=1}^{m}\tfrac{1}{|\mcal D_i|}\tsum_{j=1}^{|\mcal D_i|}-\ell(a_i^j+\zeta, b_i^j),
\end{equation}
where the dataset $\mcal D_i=\{a_i^j,b_i^j\}$, $a_i^j$ represents the image features and $b_i^j\in \mbb R^{C}$ is the  one-hot encoding label, $C$ is the number of classes, $|\mcal D_i|$ is the cardinality of dataset $\mcal D_i$, $\kappa$ is the constraint level of the distortion, $\ell(\cdot, \cdot)$ is the cross entropy function. We set $\kappa = 0.25$ for {\fashion} and $\kappa=0.5$ for {\mnist}. Following the setup in the work \cite{chen2023faster}, we iteratively perform an additional projection step for constraint satisfaction.
% \[\ell(\abf_i,b_i)=-\sum_{c=1}^{C}\log \tfrac{\exp(\mcal N(\abf_i)_c)}{\tsum_{c=1}^{C}\exp(\mcal{N}(\abf_i)_{c})}\].

\noindent\textbf{Comparison: }We use two pre-trained models with 99.29\% accuracy on {\mnist} and 92.30\% accuracy on {\fashion}, respectively. We use GFM, GFM$^{+}$, {\dgfmlin} and {\dgfm} to attack the pre-trained LeNet on $59577$ images of {\mnist} and $55384$ images of {\fashion}, which are classified correctly on the train set for training LeNet. Furthermore, we evaluate the perturbation on a dataset comprising 9885 MNIST images and 8975 Fashion-MNIST images. These images have been accurately classified during the testing phase of the LetNet training. Throughout all the experiments, we set $\delta=0.01$, $b=\{16, 32, 64\}$. For {\dgfm} and GFM$^{+}$, we tune $b^{\prime}$ from $\{40, 80, 800, 1600\}$, $T$ from $\{2, 5, 10, 20\}$. Additionally, tune $\mcal T$ from $\{1, 10, 20\}$ for {\dgfm}. For all algorithms, we tune the stepsize $\eta$ from $\{0.05, 0.1, 0.5, 1\}$ and multiply a decay factor $0.6$ if no improvement in $300$ iterations. For all experiments, we set the initial perturbation as $\zerobf$. The results of  the average of five runs are shown in Figure~\ref{fig:res_attack} and Table~\ref{tab:accuracy_attack}.  On the Fashion-MNIST dataset, {\dgfmlin} achieves the lowest accuracy after attacking and small variance. For MNIST, {\dgfm} achieves the lowest accuracy after attacking, but its variance is larger. In general, we can observe that our algorithms perform better than the serial counterparts.



==> result_fig_arxiv.tex <==
\begin{figure}[htp]
\begin{centering}
\begin{minipage}[t]{0.33\columnwidth}%
      \includegraphics[width=5.5cm]{fig/a9a.pdf}%
\end{minipage}%
\begin{minipage}[t]{0.33\columnwidth}%
\includegraphics[width=5.5cm]{fig/covtype.pdf}%
\end{minipage}%
\begin{minipage}[t]{0.33\columnwidth}%
\includegraphics[width=5.5cm]{fig/HIGGS.pdf}%
\end{minipage}
\par
\begin{minipage}[t]{0.33\columnwidth}%
\includegraphics[width=5.5cm]{fig/ijcnn.pdf}%  
\end{minipage}
\begin{minipage}[t]{0.33\columnwidth}%
\includegraphics[width=5.5cm]{fig/phishing.pdf}%    
\end{minipage}
\begin{minipage}[t]{0.33\columnwidth}%
\includegraphics[width=5.5cm]{fig/skin_nonskin.pdf}%    
\end{minipage}
\begin{minipage}[t]{0.33\columnwidth}%
\includegraphics[width=5.5cm]{fig/rcv.pdf}%    
\end{minipage}
\begin{minipage}[t]{0.33\columnwidth}%
\includegraphics[width=5.5cm]{fig/SUSY.pdf}%
\end{minipage}
\begin{minipage}[t]{0.33\columnwidth}%
\includegraphics[width=5.5cm]{fig/w8a.pdf}%    
\end{minipage}
\end{centering}
\caption{\label{fig:res}Comparison of convergence performance. $y$-axis: objective function value; $x$-axis:  number of calls to the zeroth-order oracle.}
\end{figure}
